A Novel CNet-assisted Evolutionary Level Repairer and Its Applications to Super Mario Bros

Applying latent variable evolution to game level design has become more and more popular as little human expert knowledge is required. However, defective levels with illegal patterns may be generated due to the violation of constraints for level design. A traditional way of repairing the defective levels is programming specific rule-based repairers to patch the flaw. However, programming these constraints is sometimes complex and not straightforward. An autonomous level repairer which is capable of learning the constraints is needed. In this paper, we propose a novel approach, CNet, to learn the probability distribution of tiles giving its surrounding tiles on a set of real levels, and then detect the illegal tiles in generated new levels. Then, an evolutionary repairer is designed to search for optimal replacement schemes equipped with a novel search space being constructed with the help of CNet and a novel heuristic function. The proposed approaches are proved to be effective in our case study of repairing GAN-generated and artificially destroyed levels of Super Mario Bros. game. Our CNet-assisted evolutionary repairer can also be easily applied to other games of which the levels can be represented by a matrix of objects or tiles.

==> codes/cross.tex <==
% \newcommand\repalceSet[1]{R(#1)}
% \newcommand\PCzero{$\lambda_0$}
% \newcommand\PMzero{$\sigma_0$}
% \newcommand\type[3]{T(#1, #2$\vert$#3)}


% \begin{algorithm}[htbp]
% 	\caption{Cross$(x_1, x_2)$}
% 	\begin{algorithmic}[1]
%         \State $x'_1 \gets x_1$, $x'_2 \gets x_2$
%         \For{$(i,j)$ in $R(x_1)$ $\cup$ $R(x_2)$}
%             \State At a probability of $\lambda_0$:
%             \State swap $x'_1(i,j)$ and $x'_2(i,j)$
%         \EndFor
%         \State\Return $x'_1$, $x'_2$
% 	\end{algorithmic}
% \end{algorithm}

\begin{algorithm}[htbp]
\caption{\label{algo:crossover}Crossover operator.}
\begin{algorithmic}[1]
\Function{Crossover}{$x_1, x_2$}
\State $x'_1 \gets x_1$, $x'_2 \gets x_2$
        \For{$(i,j) \in \mathcal{R}(x_1) \times \mathcal{R}(x_2)$}
            \State At a probability of $p_c$, swap $x'_1(i,j)$ and $x'_2(i,j)$
        \EndFor
        \State\Return $x'_1$, $x'_2$
\EndFunction
\Function{Mutation}{$x$}  
\State $x' \gets x$
        \For{$(i,j) \in \mathcal{S}$}
            \State At a probability of $\sigma_0$:
            \State $x'(i,j) \gets$ randomly select in $\mathcal{C}^{l}_{i,j}$
        \EndFor 
\State\Return $x'$
\EndFunction
\end{algorithmic}
\end{algorithm}

==> codes/mutation.tex <==
% \begin{algorithm}[!h]
% 	\caption{Mutation$(x)$}
% 	\begin{algorithmic}[1]
%         \State $x' \gets x$
%         \For{$(i,j)$ in $S$}
%             \State At a probability of $\sigma_0$:
%             \State $x'(i,j) \gets$ random select in $C^{l}_{i,j}$
%         \EndFor 
%         \State\Return $x'$
%  	\end{algorithmic}
% \end{algorithm}

\begin{algorithm}[htbp]
\caption{\label{algo:mutation}Mutation operator.}
\begin{algorithmic}[1]
\Function{Mutation}{$x$}  
\State $x' \gets x$

        \For{$(i,j) \in \mathcal{S}$}
            \State At a probability of $\sigma_M1$:
            \State $x'(i,j) \gets$ randomly select in $\mathcal{C}^{l}_{i,j}$
        \EndFor 
\State\Return $x'$
\EndFunction
 \end{algorithmic}
\end{algorithm}

==> codes/repair.tex <==
% \begin{algorithm}[!h]
% 	\caption{Repair$(x)$}
% 	\begin{algorithmic}[1]
%         \State $x' \gets x$
%         \For{$(i,j)$ in $U(x')$}
%             \State $x'(i,j) \gets$ random select in $C^x_{i,j}$
%         \EndFor
%         \State\Return $x'$
% 	\end{algorithmic}
% \end{algorithm}

\begin{algorithm}[htbp]
\caption{\label{algo:repair}Repair operator.}
\begin{algorithmic}[1]
\Function{Repair}{$x$}
        \State $x' \gets x$
        \For{$(i,j) \in \mathcal{U}(x')$}
            \State $x'(i,j) \gets$ randomly select in $\mathcal{C}^x_{i,j}$
        \EndFor
        \State\Return $x'$
\EndFunction
\end{algorithmic}
\end{algorithm}

==> tables/notations.tex <==
%\renewcommand\arraystretch{1.4}
\begin{table}[htbp]
        \centering
            \caption{\label{tab:notations}Some of the notations used in this paper.}
        \begin{tabular}{cl}
            \toprule
            \textbf{Notation}   & \multicolumn{1}{c}{\textbf{Meaning}}\\
            \midrule
            $l$ & The original level need to be repair\\
            \hline
            $\mathcal{S}_l$     & The set of wrong tiles and unstable tiles in a given level $l$\\
            \hline
            $\mathcal{W}(x)$     & The set of wrong tiles in a level $x$\\
            \hline 
            $\mathcal{U}(x)$     & The set of unstable tiles in a level $x$\\
            \hline 
            $\mathcal{C}^x_{i,j}$  & The set of all candidate types of a tiles at $(i,j)$ \\
            \hline
            $\mathcal{R}(x)$     & The set of replaced girds of a solution $x$\\
            \hline 
            $P(T_{i,j}=t)$     & The predict probability of type $t$ in $(i,j)$\\
            \bottomrule
        \end{tabular}
    \end{table}
